FedUMM: A General Framework for Federated Learning with Unified Multimodal Models

Unified multimodal models (UMMs) are emerging as strong foundation models that can do both generation and understanding tasks in a single architecture. However, they are typically trained in centralized settings where all training and downstream datasets are gathered in a central server, limiting the deployment in privacy-sensitive and geographically distributed scenarios. In this paper, we present FedUMM, a general federated learning framework for UMMs under non-IID multimodal data with low communication cost. Built on NVIDIA FLARE, FedUMM instantiates federation for a BLIP3o backbone via parameter-efficient fine-tuning: clients train lightweight LoRA adapters while freezing the foundation models, and the server aggregates only adapter updates. We evaluate on VQA v2 and the GenEval compositional generation benchmarks under Dirichlet-controlled heterogeneity with up to 16 clients. Results show slight degradation as client count and heterogeneity increase, while remaining competitive with centralized training. We further analyze computation--communication trade-offs and demonstrate that adapter-only federation reduces per-round communication by over an order of magnitude compared to full fine-tuning, enabling practical federated UMM training. This work provides empirical experience for future research on privacy-preserving federated unified multimodal models.

==> tables/tab-semantic.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Robustness to multimodal semantic shift.} VQA v2 accuracy (\%) under different noise injection scenarios with $K=8$, $\alpha=0.5$.}
\label{tab:noise_robustness}
\vspace{-2mm}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l|c|cc|cc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Clean}} & \multicolumn{2}{c|}{\textbf{Image Noise}} & \multicolumn{2}{c}{\textbf{Text Noise}} \\
& & 10\% & 20\% & 10\% & 20\% \\
\midrule
FedAvg &  &  &  &  &  \\
FedProx &  &  &  &  &  \\
FedOpt &  &  &  &  &  \\
\midrule
\textbf{Fed-UMLLM} &  &  &  &  &  \\
\bottomrule
\end{tabular}%
}
\vspace{-3mm}
\end{table}
